A Polynomial Time, Pure Differentially Private Estimator for Binary Product Distributions

We present the first $\varepsilon$-differentially private, computationally efficient algorithm that estimates the means of product distributions over $\{0,1\}^d$ accurately in total-variation distance, whilst attaining the optimal sample complexity to within polylogarithmic factors. The prior work had either solved this problem efficiently and optimally under weaker notions of privacy, or had solved it optimally while having exponential running times.

==> neurips23-submit/acks.tex <==
\section*{Acknowledgements}

We would like to thank Gautam Kamath for their helpful discussion on this problem.

==> neurips23-submit/intro.tex <==
\section{Introduction}

Machine learning and statistics aim to learn information about the population. The pertinent algorithms always involve using random samples from the relevant population to learn and release that information, but at the same time, often end up revealing sensitive information about the individuals in the datasets. \emph{Differential privacy (DP)} \cite{DworkMNS06} is now a \emph{de facto} standard for preserving privacy in learning and testing algorithms. It informally guarantees that no adversary can infer anything more about an individual from the output of a differentially private algorithm, than they could have from its output if the individual were not present in the dataset.

In the last few years, a large body of work on differentially private statistics has emerged, which has shown that the privacy constraint always tends to impose an additional cost in the sample complexity for those tasks (see Section~\ref{sec:intro-related}). Depending on the strength of the privacy guarantee (e.g., pure, concentrated \cite{BunS16, DworkR16}, or approximate differential privacy), the running times of the private algorithms also tend to get affected greatly. It is often the case that developing pure DP algorithms for a statistical task, which has the optimal sample complexity and a polyomial running time, is much more challenging than creating efficient and (sample) optimal, concentrated or approximate DP algorithms for the same task. For instance, mean estimation of heavy-tailed distributions in total-variation distance under pure DP was solved optimally, but without computational efficiency, in \cite{KamathSU20}, but obtaining a computationally efficient algorithm for the same remained an open problem until it was solved recently in \cite{HopkinsKM22}. On the other hand, \cite{KamathSU20} did provide computationally efficient and optimal, concentrated and approximate DP algorithms for mean estimation of heavy-tailed distributions. Similarly, \cite{KamathLSU19} presented efficient and optimal, concentrated and approximate DP algorithms for mean estimation of multivariate Gaussians, but solving this problem optimally and with computational efficiency under pure DP remained open until \cite{HopkinsKMN23} solved it recently.

Estimating binary product distributions (product distributions over $\zo^d$) in total-variation distance is another such example. In this case, too, optimal and computationally efficient, concentrated and approximate DP algorithms had been presented already in \cite{KamathLSU19}, but no computationally efficient and optimal, pure DP algorithm was known after that, although multiple optimal algorithms for this problem under pure DP, but lacking the computational efficiency, have come up in the recent past (e.g., \cite{BunKSW19}). In this work, we provide an optimal and a computationally efficient algorithm that satisfies pure DP, and close that gap for this problem.

\subsection{Estimation in Total-Variation Distance}
    \label{sec:intro-challenges}

We would first like to remind the reader as to why estimating binary product distributions in total-variation distance is a much more difficult task than just simply estimating them in $\ell_2$ distance. A small error in total-variation distance requires all the marginals to be estimated accurately with respect to the magnitudes of their respective means, that is, the error for each marginal needs to be scaled according to the magnitude of its mean. In certain situations, it could imply that each marginal needs to be estimated to within a small multiplicative error. Instead, if in the estimate, all the coordinates have similar additive errors, then unless that error is \emph{very} small, the marginals with very small means would have significantly lower accuracy than the ones with much larger means. Therefore, the estimate would not be accurate in total-variation distance. On the other hand, if we have the additive errors to be very small for all the coordinates (say, if we are estimating the distribution to within $\ell_1$ distance $\alpha$ or to within $\ell_{\infty}$ distance $\tfrac{\alpha}{d}$), then the cost of estimation would become very large in terms of the sample complexity. Therefore, we need to find a way to estimate product distributions accurately \emph{direction-wise}.

Sans privacy, this is an easy task -- we can just output the empirical mean of the samples. Under privacy constraints, however, this is hard to do without knowing even an approximate scale of the noise to add in each direction. The na\"{i}ve way to estimate privately would just involve either adding a very small noise to each coordinate of the empirical mean, but that would increase the cost in the sample complexity dramatically (by $\poly(d)$). On the other hand, even if we use a sophisticated pure DP estimator, which simply estimates accurately in $\ell_2$ distance $\alpha$, this would not be accurate enough either. Thus, we need more non-trivial ways to privately estimate each coordinate to within an error that is scaled appropriately for that marginal.

\subsection{Result}

We informally state the main result of this work here. It essentially says that our pure DP algorithm is computationally efficient and estimates the mean of any product distribution over $\zo^d$ in total-variation distance using just $\wt{O}(d)$ samples.

\begin{thm}[Informal]\label{thm:ppde-informal}
    For every $\eps,\alpha,\beta > 0$, there exists a
    polynomial-time, $\eps$-DP algorithm that takes $n$ i.i.d.\ samples from a product distribution $P$ over $\zo^d$, and returns a product distribution $Q$, such that if
    $n \geq \wt{O}\left(
        \tfrac{d}{\alpha^2} + \tfrac{d}{\eps\alpha}\right)$,
    where $\wt{O}(\cdot)$ hides all polylogarithmic factors,
    then with probability at least $1-\beta$, the total-variation distance between $P$ and $Q$ is at most $\alpha$.
\end{thm}

Note that this is the optimal sample complexity for this problem, and the upper bounds under approximate DP and the matching lower bounds (which also hold under pure DP) were proved in \cite{KamathLSU19}. The first term in the sample complexity is the necessary term for attaining the desired accuracy without any privacy constraints, and the second term is the additive cost due to privacy. For $\eps \geq \Omega(\alpha)$, privacy comes for ``free'', that is, there is only a small multiplicative cost in the non-private sample complexity. Additionally, as we will see in the formal version of the above theorem (see Theorem~\ref{thm:ppde}), there is also a multiplicative $\polylog(d,\tfrac{1}{\beta},\tfrac{1}{\eps})$ improvement in the sample complexity over that of \cite{KamathLSU19} due to our tighter analysis.

\subsection{Overview of Techniques}

Our techniques are similar to those in \cite{KamathLSU19} for estimating binary product distributions -- private partitioning, followed by privately estimating. Before we provide a brief outline of our algorithm, we would like to note its two important aspects.
\begin{itemize}
    \item In the partitioning procedure, we filter out the ``heavier'' marginals iteratively, and group the ones with similar weights together, but unlike the algorithm in \cite{KamathLSU19}, ours does not estimate them simultaneously while the partitioning is being performed. This is because we wanted to avoid the additional $\poly(d)$ cost in the sample complexity due to (basic) composition under pure DP. However, \cite{KamathLSU19} were able to both partition and estimate those heavy marginals at the same time because they were working under concentrated or approximate DP, and they could use the more sophisticated, advanced composition of privacy \cite{DworkRV10}, which only provides concentrated or approximate DP guarantees.
    \item In order to estimate those heavier marginals after filtering and grouping them, we rescale them using their respective rough private estimates that we obtained while partitioning, and apply the pure DP sub-Gaussian mean estimator from \cite{HopkinsKMN23}, which is computationally efficient, as well. This gives us an estimate of the scaled marginals that is accurate to within $\alpha$ in $\ell_2$ distance.
\end{itemize}

The private partitioning is performed iteratively. In each round, we assume an upper bound on the marginals, and use the Laplace mechanism (scaled according to that upper bound and the number of marginals that remain to be partitioned) to get a rough private estimate of each marginal, and pick the ones that lie above a certain threshold. As we prove later, those coordinates are bound to have higher means than the ones with their noisy estimates below that threshold. We rescale those chosen heavier coordinates as per the assumed upper bound for that iteration, and mark them to be estimated later after the partitioning is complete. In the next round, we assume both a reduced upper bound on the marginals and a reduced threshold to filter out the next set of marginals, and repeat the process.

Once we have filtered and rescaled those heavier marginals, we estimate them in $\poly(n,d)$ time to within $\alpha$ in $\ell_2$ distance under pure DP using the sub-Gaussian learner from \cite{HopkinsKMN23}. On inverse-rescaling the estimated marginals according to their respective original rescaling parameters, we get an accurate estimate for those heavier coordinates to within $O(\alpha)$ in total-variation distance. Note that we cannot simply invoke the estimator from \cite{HopkinsKMN23} on the filtered out coordinates before rescaling them, since that would just give an $\ell_2$ estimate of the original marginals, which would not be accurate direction-wise, hence, would not be accurate in total-variation distance, especially when there are marginals with very different magnitudes in that filtered set (see Section~\ref{sec:intro-challenges}). Therefore, this combination of partitioning and rescaling those heavier marginals seems necessary for this kind of an approach.

After the partitioning rounds, we have the final round, where we are just left with the lighter coordinates to estimate. For that, we simply use the Laplace mechanism again, but with a much lower sensitivity this time, and get an accurate estimate for those marginals directly in one shot.

With accurate estimates for both the heavy and the light marginals in hand, we finally combine the two via a simple concatenation, and this gives us an accurate estimate for the whole distribution, as we had originally desired.

\subsection{Related Work}\label{sec:intro-related}

Besides a large selection of folklore work in non-private estimation of distributions, there has been a lot of work in recent years on differentially private statistical estimation.
Mean estimation is possibly the most fundamental question in this space, enjoying significant attention (e.g.,~\cite{BarberD14, DuchiJW13, KarwaV18, BunS19, KamathLSU19, KamathSU20, WangXDX20, DuFMBG20, BiswasDKU20, CaiWZ21, BrownGSUZ21, HuangLY21, LiuKKO21, LiuKO22, KamathLZ22, HopkinsKM22, KothariMV22, TsfadiaCKMS22, DuchiHK23, CovingtonHHK21, NikolovT23, KamathMRSSU23}).
Other related problems include private covariance or density estimation~\cite{BunNSV15, BunKSW19,AdenAliAK21,KamathMSSU22, AshtianiL22, AlabiKTVZ22,HopkinsKMN23, KothariMV22, TsfadiaCKMS22, LiuKO22, BiswasDKU20}.
Beyond these settings, other works have examined statistical estimation under differential privacy constraints for mixtures of Gaussians~\cite{KamathSSU19, AdenAliAL21,ChenCDEIST23}, graphical models~\cite{ZhangKKW20}, discrete distributions~\cite{DiakonikolasHS15}, median estimation~\cite{AvellaMedinaB19, TzamosVZ20,RamsayC21,RamsayJC22,BenEliezerMZ22, CummingsD20}, and more.
Several recent works have explored the connections between privacy and robustness \cite{LiuKKO21, HopkinsKM22, GeorgievH22, LiuKO22, KothariMV22, AlabiKTVZ22, HopkinsKMN23,ChenCDEIST23}, and between privacy and generalization \cite{HardtU14,DworkFHPRR15,SteinkeU15,BassilyNSSSU16,RogersRST16,FeldmanS17}.
Upcoming directions of interest include ensuring privacy when one individual may contribute multiple data points \cite{LiuSYKR20, LevySAKKMS21, GeorgeRST22} (or what is known as, \emph{user-level differential privacy}), a combination of local and central DP for different users~\cite{AventDK20}, and estimation with access to trace amounts of public data~\cite{BieKS22}.
We refer the reader to \cite{KamathU20} for more coverage of the recent work on differentially private statistical estimation.
Differentially private statistical inference also has been an active area of research for over a decade (e.g., \cite{DworkL09, VuS09, WassermanZ10, Smith11}), but the literature is too broad to fully summarize here.

The two prior works most relevant to ours among the above are those by \cite{KamathLSU19, HopkinsKMN23} on learning binary product distributions under concentrated and approximate DP, and estimating means of sub-Gaussian distributions under pure DP, respectively. The question of learning binary product distributions optimally in polynomial time under pure DP has stayed open for a while now. In our work, we modify and use a combination of their techniques to solve this problem.

\subsection{Organization}

We start by stating a few statistical notations and some basic background in differential privacy in Section~\ref{sec:prelims}. In Section~\ref{sec:product}, we provide our main algorithm and the relevant theoretical results and proofs. We provide some additional related work in differentially private statistical estimation in Appendix~\ref{sec:related-extra}. The other necessary statistical and privacy preliminaries are stated in Appendix~\ref{sec:prelims-app}. We include the missing proofs from Section~\ref{sec:product} in Appendix~\ref{sec:missing-proofs}.

==> neurips23-submit/prelims.tex <==
\section{Preliminaries}\label{sec:prelims}

For the utility analysis, we mostly rely on the concentration properties of Bernoulli distributions and the Laplace distribution, and on the relationships among different distance metrics for probability distributions. The privacy analysis is much simpler, and we use the privacy guarantees of the existing differentially private mechanisms. We describe some of these notions and results in this section.

\subsection{Statistics Preliminaries}

Here, we state a few essential notations from
statistics that would be used throughout the draft.
Other relevant preliminaries could be found in
Appendices~\ref{sec:prelims-distances} and~\ref{sec:prelims-tb}.

\paragraph{Notations.} Let $P_1,\dots,\P_k$ be distributions over domains $\cX_1,\dots,\cX_k$, respectively. Then we say that $P=P_1\otimes\dots\otimes P_k$ is a product distribution over $\cX_1\otimes\dots\otimes\cX_k$. Next, for a distribution $P$ over domain $\cX$, we use $P^{\otimes k} = P\otimes\dots\otimes P$ ($k$ times) to denote the product distribution over $\cX\otimes\dots\otimes\cX$ ($k$ times), where each marginal is $P$.
Also, for $0\leq p \leq1$, we use $\Ber(p)$ to denote a Bernoulli random variable with mean $p$.
Finally, for any $v=(v_1,\dots,v_d) \in \R^d$, we use $\abs{v}$ to denote its $\ell_1$ norm, i.e., $\abs{v} = \sum\limits_{i=1}^{d}{\abs{v_1}}$.

\subsection{Privacy Preliminaries}

We start with the definition of differential privacy.
\begin{defn}[Differential Privacy (DP) \cite{DworkMNS06}]
    \label{def:dp}
    A randomized algorithm $M:\cX^n \rightarrow \cY$
    satisfies $(\eps,\delta)$-differential privacy
    ($(\eps,\delta)$-DP) if for every pair of
    neighboring datasets $X,X' \in \cX^n$
    (i.e., datasets that differ in at most one entry, denoted by $X \sim X'$),
    $$\forall~ Y \subseteq \cY,~~~
        \pr{}{M(X) \in Y} \leq e^{\eps}\cdot
        \pr{}{M(X') \in Y} + \delta.$$
    When $\delta = 0$, we say that $M$ satisfies
    $\eps$-differential privacy or pure differential
    privacy.
\end{defn}

\noindent These definitions of DP are closed under post-processing.
\begin{lem}[Post-Processing \cite{DworkMNS06}]\label{lem:post-processing}
    If $M:\cX^n \rightarrow \cY$ is
    $(\eps,\delta)$-DP, and $P:\cY \rightarrow \cZ$
    is any randomized function, then the algorithm
    $P \circ M$ is $(\eps,\delta)$-DP.
\end{lem}

\begin{comment}
\begin{lem}[Composition of DP~\cite{DworkMNS06}]\label{lem:composition}
    Suppose $M$ is an adaptive composition of
    algorithms $M_1,\dots,M_T$, which are
    $(\eps_1,\delta_1),\dots,(\eps_T,\delta_T)$-DP, respectively.
    Then $M$ is $(\eps,\delta)$-DP for
    $$\eps = \sum_t \eps_t~~~~\textrm{and}~~~~\delta = \sum_t \delta_t.$$
\end{lem}
\end{comment}

\noindent We finally state the result from \cite{HopkinsKMN23} about
estimating the means of sub-Gaussian distributions under
pure DP in polynomial time.
\begin{thm}[Sub-Gaussian Learner from {\cite[Theorem~5.1]{HopkinsKMN23}}]\label{thm:sg-learner}
    Assume that $0<\alpha,\beta,\eps<1$ and $R>0$.
    Let $\mu \in \R^d$, where $\|\mu\|_2 \leq R$, be unknown.
    There exists an $\eps$-DP algorithm ($\DPSGLearner$)
    that takes $n$
    i.i.d.\ samples from a sub-Gaussian distribution
    with mean $\mu$ and covariance $0 \preceq \Sigma \preceq \id$,
    such that,
    $n \geq
        \wt{O}_{\alpha}\left(\tfrac{d + \log(1/\beta)}{\alpha^2}
            + \tfrac{d + \log(1/\beta)}{\alpha \eps}
            + \tfrac{d\log(R)}{\eps}\right)$,
    where $\wt{O}_{\alpha}(\cdot)$ hides polylogarithmic factors
    in $\tfrac{1}{\alpha}$, runs in time $\poly(n,d)$,
    and with probability at least $1-\beta$, outputs
    $\wh{\mu}$ such that $\|\mu - \wh{\mu}\|_2 \leq \alpha$.
\end{thm}

==> neurips23-submit/prod-dists.tex <==
\section{A Pure DP Product Distribution Estimator}
\label{sec:product}

In this section we introduce and analyze our algorithm for learning a product distribution $P$ over $\zo^d$ in total-variation distance. The pseudocode is stated in Algorithm~\ref{alg:ppde}, with some additional observations and information regarding the notations stated in Section~\ref{sec:algorithm}. For simplicity of presentation, we assume that the product distribution has mean, whose marginals are bounded by $\frac12$ (i.e., $\ex{}{P} \preceq \frac12$), however, we would like to clarify that this assumption is essentially without loss of any generality, and is easily removable at the cost of a meagre constant factor in the sample complexity.
We make an additional assumption that
$d \geq 2$ and that $\beta \leq \tfrac{1}{2}$.

The following is the main result of our work. We prove the privacy, the computational efficiency, and the accuracy guarantees of our algorithm in Appendices~\ref{sec:privacy}, \ref{sec:efficiency}, and Section~\ref{sec:accuracy}, respectively.
\begin{thm}\label{thm:ppde}
    For every $\eps,\alpha,\beta > 0$, there exists an $\eps$-DP algorithm ($\PPDE$) that takes $n$ i.i.d.\ samples from a product distribution $P$ over $\zo^d$, and returns a product distribution $Q$ over $\zo^d$ in $\poly(n,d,\tfrac{1}{\eps},\tfrac{1}{\alpha},\log(\tfrac{1}{\beta}))$ time, such that if
    $$n \geq \wt{O}_{\alpha}\left(
        \frac{d\log^2(d/\beta)}{\alpha^2} +
        \frac{d\log^2(d/\eps\beta)}{\eps\alpha}\right),$$
    where $\wt{O}_{\alpha}(\cdot)$ hides polylogarithmic factors
    in $\tfrac{1}{\alpha}$,
    then with probability at least $1-\beta$, $\SD(P,Q) \leq \alpha$.
\end{thm}

\subsection{The Algorithm}\label{sec:algorithm}

We first introduce a notation for the \emph{truncated mean} of all the points in a dataset. Given a data point $x \in \zo^{d}$ and $B \geq 0$, we write
\begin{equation*}
\trunc_{B}(x) = 
\begin{cases}
x &\textrm{if $\abs{x} \leq B$}\\
\frac{B}{\abs{x}} \cdot x &\textrm{if $\abs{x} > B$}
\end{cases}
\end{equation*}
to denote the truncation (or clipping) of $x$ to an $\ell_1$-ball of radius $B$.  Given a dataset $X = (X_1,\dots,X_{m}) \in \zo^{m \times d}$ and $B > 0$, we use
$$
\tmean_{B}(X) = \frac{1}{m} \sum_{i=1}^{m} \trunc_{B}(X_i)
$$
to denote the mean of the truncated data points in $X$.
If one of the data points in $X$ does not satisfy
the norm bound (i.e., its $\ell_1$ norm is greater than $B$) when $X$ is served as an input to $\tmean_B$, then we will say,
``truncation occurred,'' as a shorthand.
We point out a couple of important observations.
\begin{itemize}
    \item The $\ell_1$-sensitivity of $\tmean_{B}$ is $\frac{B}{m}$, while the $\ell_1$-sensitivity of the un-truncated mean is $\tfrac{d}{m}$.
    \item Unless $\abs{X_{i}} > B$ for some $i \in [m]$, the truncated mean equals the un-truncated mean, i.e., $\tmean_{B}(X) = \frac{1}{m} \sum_{i=1}^{m} X_{i}$.
\end{itemize}

We also use the following notational conventions.
Given a data point $X_i \in \zo^d$, we use $X_i[j]$ to refer to its $j$-th coordinate, and for a subset of coordinates $S \subseteq [d]$, the notation $X_i[S] = (X_i[j])_{j \in S}$ to refer to the vector $X_i$ with coordinates restricted to $S$. Given a dataset $X = (X_1,\dots,X_m)$, we use the notation $X[S] = (X_1[S],\dots,X_m[S])$ to refer to the dataset consisting of each $X_i[S]$.
Next, for a domain $\cX$, a variable $x \in \cX$, and a probability distribution $D$ over $\cX$, we write ``$x \gets_R D$'' to indicate that a sample has been drawn from $D$, and assigned to $x$.
Finally, in Algorithm~\ref{alg:ppde}, we use $C_{\alpha}$ to denote the $\polylog(1/\alpha)$ quantity in the sample complexity from Theorem~\ref{thm:sg-learner}.

\begin{algorithm}[h!] \label{alg:ppde}
\caption{Pure DP Product Distribution Estimator $\PPDE_{\eps, \alpha, \beta}(X)$}
\KwIn{Samples $X_1,\dots,X_n \in \zo^{d}$ from an unknown product distribution $P$ satisfying $\ex{}{P} \preceq \frac12$.  Parameters $\eps, \alpha, \beta > 0$.}
\KwOut{A product distribution $Q$ over $\{0,1\}^d$ such that $\SD(P,Q) \leq \alpha$.}\vspace{10pt}
Set parameters:
$
R \gets \log_{2}\left(d/2\right)~~~
m \gets 2048 d \log(d/\beta) + \tfrac{2048 d \log(d/\eps\beta)}{\eps}
$\\
$
\qquad \qquad \qquad~~ m_0 \gets C_{\alpha}\left(\tfrac{d+\log(1/\beta)}{\alpha^2} + \tfrac{d+\log(1/\beta)}{\alpha\eps} + \tfrac{d\log(d)}{\eps}\right)$\\
$
\qquad \qquad \qquad~~ m_1 \gets \tfrac{128d\log(d/\beta)}{\alpha^2} + \tfrac{256d\log(d/\eps\alpha\beta)}{\eps\alpha}
$\\
\vspace{10pt}

Split $X$ into three datasets $Y$, $Y_F$, and $Z$, of sizes $mR$, $m_1$, and $m_0$, respectively.\\
Split $Y$ into $R$ blocks $Y^1,\dots,Y^R$ of sizes $m$ each, denoted by $Y^{r} = (Y^{r}_{1},\dots,Y^{r}_{m})$.\\
Let $q \in (0,1)^d$ with $q[j] \gets 0$ for all $j \in [d]$, and let $S_1 = [d]$, $u_1 \gets \frac{1}{2}$, $\tau_1 \gets \frac{3}{16}$, and $r \gets 1$.\\
\vspace{10pt}

\tcp{Partitioning rounds.}
Let $T_P \gets \emptyset$.\\
\While{$u_r \abs{S_r} \geq 1$ and $r \leq R$}{
    Let $S_{r+1}, T_r \gets \emptyset$.\\
    Let $B_r \gets 3 u_r |S_r| \log(mR/\beta)$.\\
    Let $z_r \getsr \Lap\left(\tfrac{B_r}{\eps}\right)^{\otimes \abs{S_r}}$ and $q_r[S_r] \gets \tmean_{B_r}(Y^r[S_r]) + z_r$.\\
    \For{$j \in S_r$}{
        \eIf{$q_r[j] < \tau_r$}{
            Add $j$ to $S_{r+1}$.
            }
            {
            Add $j$ to $T_{r}$.
            }
    }
    Set $Z[T_r] \gets \tfrac{1}{\sqrt{u_r}}\cdot Z[T_r]$.\\
    Set $T_P \gets T_P \cup T_r$.\\
    \tcp{Update the loop's parameters.}
    Set $u_{r+1} \gets \frac12 u_{r}$, $\tau_{r+1} \gets \frac12 \tau_{r}$, and $r \gets r+1$.
}
\tcp{Run the sub-Gaussian learner from \cite{HopkinsKMN23} restricted to $T_P$.}
Let $\wh{q}[T_P] \getsr \DPSGLearner_{\eps,\frac{\alpha}{5},\beta,\sqrt{d}}(Z[T_P])$.\\
\For{$i \in [r-1]$}{
    Set $q[T_i] \gets \sqrt{u_i}\cdot\wh{q}[T_i]$.
}
\vspace{10pt}
    
\tcp{Final round.}
Let $S_F \gets [d] \setminus T_P$.\\
\If{$\abs{S_F} \geq 1$}{
    Let $B_F \gets 4\log(m_1/\beta)$.\\
    Let $z \getsr \Lap\left(\tfrac{B_F}{\eps}\right)^{\otimes \abs{S_F}}$ and $q[S_F] \gets \tmean_{B_F}(Y^F[S_F]) + z$.
}
\vspace{10pt}

\tcp{Return the final estimate.}
\Return $Q = \Ber(q[1]) \otimes \dots \otimes \Ber(q[d])$.
\end{algorithm}

\subsection{Accuracy Analysis}\label{sec:accuracy}

In this section we prove the following proposition bounding the sample complexity required by \PPDE{} to be accurate.

\begin{prop}\label{thm:ppde_acc}
    For every $d \in \N$, every product distribution
    $P$ over $\zo^{d}$, and every $\eps,\alpha, \beta > 0$,
    if $X = (X_1,\dots,X_n)$ are independent samples
    from $P$, where
    $
        n \geq \wt{O}_{\alpha}\left(\tfrac{d\log^2(d/\beta)}{\alpha^2}
        + \tfrac{d\log^2(d/\eps\beta)}{\alpha\eps}\right)
    $,
    then with probability at least $1-O(\beta)$,
    $\PPDE_{\eps,\alpha,\beta}(X)$ outputs $Q$,
    such that $\SD(P,Q) \leq \alpha$. The notation $\wt{O}_{\alpha}(\cdot)$ hides polylogarithmic factors in $\tfrac{1}{\alpha}$.
\end{prop}

\subsubsection{Analysis of the Partitioning Rounds}

In this section we analyze the progress made during the partitioning rounds.  We show two properties for any round $r$: (1) any coordinate $j$ such that $q_r[j]$ was filtered out during the partitioning rounds has a large mean, and (2) any coordinate $j$, such that $q_r[j]$ was moved on to the next round, has a small mean. We capture the properties of the partitioning rounds that will be necessary for the proof of Theorem~\ref{thm:ppde_acc} in the following lemma.

\begin{lem}[Partitioning Rounds]\label{lem:ppde_partitioning}
    If $Y^{1},\dots,Y^{R}$ each contain at least
    $
    m \geq 2048 d \log(d/\beta)
        + \tfrac{2048 d \log(d/\eps\beta)}{\eps}
    $
    i.i.d.\ samples from $P$, and $Z$ contains
    $m_0 \geq \wt{O}_{\alpha}\left(\tfrac{d + \log(1/\beta)}{\alpha^2} + \tfrac{d + \log(1/\beta)}{\alpha\eps} + \tfrac{d\log(d)}{\eps}\right)$
    i.i.d.\ samples from $P$ (where $\wt{O}_{\alpha}(\cdot)$ hides polylogarithmic factors in $\tfrac{1}{\alpha}$),
    then with probability at least $1-O(\beta)$,
    in every partitioning round $r \in [R]$, we have the following.
    \begin{enumerate}
        \item If a coordinate $j$ is filtered out in round $r$ (i.e., $q_r[j] \geq \tau_r$), then $p[j]$ is large: 
            $
                p[j] \geq \tfrac{15\tau_r}{17}
            $.
        \item If a coordinate $j$ is not filtered out in round $r$ (i.e., $q_r[j] < \tau_r$), then
            $p[j]$ is small:
            $
                p[j] \leq u_{r+1} = \frac{u_{r}}{2}
            $.
    \end{enumerate}
    Therefore, if $S_P \subseteq [d]$ is the set of all the coordinates estimated in the partitioning rounds, then with probability at least $1-O(\beta)$, $\SD(P[S_P],Q[S_P]) \leq \tfrac{\alpha}{2}$.
\end{lem}
\begin{proof}
We will prove the lemma by induction on $r$.
Therefore, we will assume that
in every round $r$, $p[j] \leq u_{r}$ for
every $j \in S_{r}$ and prove that if this
bound holds, then the two claims in the
lemma hold. For the base of the induction,
observe that, by assumption, $p[j] \leq u_{1} = \frac12$
for every $j \in S_{1} = [d]$.  In what
follows we fix an arbitrary round $r \in [R]$.
Throughout the proof, we will use the notation
$\tilde{p}_{r} = \frac{1}{m} \sum_{i = 1}^{m} Y^{r}_{i}$
to denote the empirical mean of the $r$-th
block of samples.

\begin{clm}[Sampling Error in Partioning Rounds]\label{clm:part-samp-err}
    If $\tilde{p}_r[j] = \frac{1}{m} \sum_{i=1}^{m} Y^{r}_{i}[j]$ and
    $m \geq 1024d\log(dR/\beta)$, then
    with probability at least $1-\frac{2\beta}{R}$,
    $
        \forall j \in S_{r}~~\left| p[j] - \tilde{p}_r[j] \right|
        \leq \sqrt{\tfrac{4p[j]
        \log\left( \frac{dR}{\beta} \right)}{m}}
    $.
    Furthermore, if $p[j] \geq \frac{1}{d}$, then
    $\left| p[j] - \tilde{p}_r[j] \right|
        \leq \tfrac{p[j]}{16}$.
\end{clm}

\begin{clm}[No Truncation in Partioning Rounds]\label{clm:part-no-trunc}
    In round $r$, with probability at least $1-\frac{\beta}{R}$,
    for every $Y^{r}_{i} \in Y^{r}$, we have that
    $\abs{Y^{r}_{i}} \leq B_{r}$.
    So, no rows of $Y^{r}$ are truncated while
    computing $\tmean_{B_{r}}(Y^{r})$.
\end{clm}
    
\begin{clm}[Error due to Privacy in Partioning Rounds]\label{clm:part-priv-err}
With probability at least $1-\frac{2\beta}{R}$,
$
    \forall j \in S_{r}~~\left| \tilde{p}_r[j] - q_{r}[j] \right| \leq
	\tfrac{3 u_r |S_r|
	\log\left(\frac{mR}{\beta}\right)
        \log\left(\frac{dR}{\beta}\right)}{\eps m}
$.
\end{clm}

Applying the triangle inequality and simplifying, using our choice of $m$, and noting that in our algorithm, $\tau_r = \tfrac{3u_r}{8}$,
we get that in each round $r$, with probability at least $1-\tfrac{4\beta}{R}$,
\begin{align}
\abs{p[j] - q_r[j]} &\leq \sqrt{\frac{4p[j]
            \log\left( \frac{dR}{\beta} \right)}{m}} +
            \frac{3 u_r |S_r|
	   \log\left(\frac{mR}{\beta}\right)
            \log\left(\frac{dR}{\beta}\right)}{\eps m}\nonumber\\
        &\leq \frac{p[j]}{16} + \frac{3u_r}{128}\label{eq:part-err1}\\
        &= \frac{p[j]}{16} + \frac{\tau_r}{16}.\label{eq:part-err2} 
\end{align}
To simplify our calculations, we will define $e_{r,j}$ to be the quantity on the right-hand-side of Inequality~\ref{eq:part-err2}.

\begin{comment}
Next, we bound the coordinate-wise $\chi^2$-divergence between $p$ and our estimate $q_r$ in round $r$.
\begin{clm}\label{clm:part-chi-ub}
    For all $j \in S_r$, with probability,
    at least, $1-\frac{4\beta}{R}$,
    $$\chi^2\left(p[j],q_r[j]\right) \leq
        \frac{4(p[j]-q_r[j])^2}{q_r[j]}.$$
\end{clm}
\begin{proof}
    For every $r$, $d$ more than some absolute constant, and
    our choice of $m$,
    $\abs{e_{r,j}} \leq \frac{1}{4},$. Also, by assumption, $p[j] \leq \frac{1}{2},$
    for all $j \in [d]$. Therefore, for
    every $r$, and every $j \in S_r$,
    \begin{align*}
        \chi^2\left(p[j],q_r[j]\right) =&~
            \frac{(p[j]-q_r[j])^2}{q_r[j]} + \frac{(p[j]-q_r[j])^2}{1-q_r[j]}\\
            =&~ \frac{(p[j]-q_r[j])^2}{q_r[j](1-q_r[j])}\\
            \leq&~ \frac{4(p[j]-q_r[j])^2}{q_r[j]}.
    \end{align*}
    This proves our claim.
\end{proof}
\end{comment}

\begin{clm}[Noisy Estimates above Threshold]\label{clm:part-above-thresh}
    With probability at least
    $1-\frac{4\beta}{R}$,
    for every $j \in S_{r}$,
    $q_{r}[j] \geq \tau_{r} \implies
        p[j] \geq \tfrac{15\tau_r}{17}$.
\end{clm}
\begin{proof}
    We know that $\abs{p_j-q_r[j]} \leq e_{r,j}$ with
    high probability, which implies that $p[j] \geq q_r[j]-e_{r,j}$.
    Now, given that $q_r[j] \geq \tau_r$ and the bound on $e_{r,j}$ from Inequality~\ref{eq:part-err2}, we have the following.
    $$p[j] \geq q_r[j] - e_{r,j} \geq \tau_r - \frac{p[j]}{16} - \frac{\tau_r}{16} \implies p[j] \geq \frac{15\tau_r}{17}$$
    This completes the proof.
\end{proof}

\begin{clm}[Noisy Estimates below Threshold]\label{clm:part-below-thresh}
    With probability at least $1-\frac{4\beta}{R}$,
    for every $j \in S_{r}$,
    $
    q_{r}[j] < \tau_{r} \Longrightarrow p[j] \leq u_{r+1} = \tfrac{u_{r}}{2}
    $.
\end{clm}
\begin{proof}
    We know that with high probability,
    $p_j \leq q_r[j] + e_{r,j}$. But since
    $q_r[j] < \tau_j$, we know that
    $p[j] < \tau_r + e_{r,j}$. Also,
    we set $\tau_r = \frac{3}{4}u_{r+1}$ in our algorithm.
    Using the bound on $e_{r,j}$ from Inequality~\ref{eq:part-err1}, this gives us the following.
    $$p[j] < \tau_r + e_{r,j} \leq \frac{3u_{r+1}}{4} + \frac{p[j]}{16} + \frac{3u_r}{128} = \frac{3u_{r+1}}{4} + \frac{p[j]}{16} + \frac{3u_{r+1}}{256} \implies p[j] \leq \frac{13u_{r+1}}{16} < u_{r+1} = \frac{u_r}{2}$$
    Our proof is complete.
\end{proof}

Claim~\ref{clm:part-below-thresh} completes the
inductive step of the proof. It establishes
that at the beginning of round $r+1$, $p_j \leq u_{r+1}$
for all $j \in S_{r+1}$.

Finally, we analyse the accuracy of the coordinates
collected in $T_P$ over all the partitioning rounds
by the call to $\DPSGLearner$.
We can bound the total-variation distance between $P[S_P]$
and $Q[S_P]$ by computing the $\chi^2$ divergence between
the two. We make two key observations here.
\begin{itemize}
    \item In round $r$, we scale $Z[T_r]$ by $\tfrac{1}{\sqrt{u_r}}$, which means that the (scaled product) distribution of that subset of the coordinates (denoted by $\wh{P}[T_r]$) is over $\left\{0,\tfrac{1}{\sqrt{u_r}}\right\}$. Let $\Sigma_{T_r}$ be its covariance matrix. Then we can observe that the eigenvalues of $\Sigma_{T_r}$ lie between $\tfrac{\tau_r(1-\tau_r)}{u_r} = \tfrac{3(1-\frac{3u_r}{8})}{8} \geq \tfrac{39}{64}$ and $\tfrac{u_r(1-u_r)}{u_r} = 1-u_r \leq 1$. Since this is true for any $r$, this must be true for the entire $\wh{P}[T_P]$, as well.
    \item Let the output product distribution from invoking $\DPSGLearner$ on $Z[T_P]$ be $\wh{Q}[T_P]$ (which has mean $\wh{q}[T_P]$). Suppose the covariance matrix of $\wh{P}[T_P]$ is $\Sigma_{P_P}$, and the value of $r$ before the update in the end of the final iteration of the \textbf{While}-loop was $r^*$. Then from Theorem~\ref{thm:sg-learner} (accuracy guarantees of $\DPSGLearner$) and our setting of the accuracy parameters in the call to $\DPSGLearner$ in Algorithm~\ref{alg:ppde}, with probability at least $1-\beta$, the squared $\ell_2$ distance between $\wh{P}[T_P]$ and $\wh{Q}[T_P]$ is given by,
    \begin{align*}
        \frac{\alpha^2}{25} &\geq \|\wh{q}[T_P]-\wh{p}[T_P]\|_2^2\\
            &= \sum\limits_{i \in [r^*]}{\|\wh{q}[T_i]-\wh{p}[T_i]\|_2^2}\\
            &= \sum\limits_{i \in [r^*]}{\frac{\|q[T_i]-p[T_i]\|_2^2}{u_i}}\\
            &= \sum\limits_{i \in [r^*]}{\frac{3\|q[T_i]-p[T_i]\|_2^2}{8\tau_i}}\tag{$\tau_i = \tfrac{3u_i}{8}$}\\
            &\geq \sum\limits_{i \in [r^*]}{\sum\limits_{j \in T_i}{\frac{45\cdot(q[j]-p[j])^2}{136\cdot p[j]}}}\tag{Claim~\ref{clm:part-above-thresh}}\\
            &= \frac{45}{544}\cdot\sum\limits_{j \in T_P}{\frac{4(q[j]-p[j])^2}{p[j]}}.
    \end{align*}
    On rearranging the above, this implies that,
    $\sum\limits_{j \in T_P}{\tfrac{4(q[j]-p[j])^2}{p[j]}} \leq \tfrac{\alpha^2}{2}$.
\end{itemize}
The above, on combining with Lemmata~\ref{lem:chi-ub}, \ref{lem:sd-ub}, and~\ref{lem:pinsker}, implies that $\dtv(P[T_P],Q[T_P]) \leq \tfrac{\alpha}{2}$.

Now, we can take the union bound over all the failure events in all the rounds and over the failure of $\DPSGLearner$, so that the conclusions of Lemma~\ref{lem:ppde_partitioning} hold with probability $1-5\beta$.
This completes the proof.
\end{proof}

\subsubsection{Analysis of the Final Round}

In this section we show that the TV error of the coordinates $j$, such that $q[j]$ was set in the final round, is small.

\begin{lem}[Final Round]\label{lem:ppde_final}
    In the final round, let $k \in [R+1]$ for which
    $u_k |S_k| < 1$. If $p[j] \leq u_k$
    for every $j \in S_{F}$, and $Y^{F}$
    contains at least
    $
    m_1 =  \tfrac{128 d \log (d/\beta )}{\alpha^2} +
        \tfrac{256 d \log(d/\eps\alpha\beta)}{\alpha\eps}
    $
    i.i.d.\ samples from $P$, then with
    probability at least $1-O(\beta)$,
    then $\SD(P[S_F], Q[S_F]) \leq \tfrac{\alpha}{2}$.
\end{lem}
\begin{proof}
    Again, we use the notation,
    $\tilde{p} = \frac{1}{m_1} \sum_{i = 1}^{m_1} Y^{F}_{i}$,
    for the rest of this proof. First, we have
    two claims that bound the difference
    between $p[j]$ and $\tilde{p}[j]$.
    
    \begin{clm}[Sampling Error for Large Coordinates in Final Round]\label{clm:final-samp-err-lrg}
        For each $j \in S_F$, such that $p_j > \frac{1}{d}$,
        with probability at least $1-2\beta/d$,
        we have,
        $
        \left| p[j] - \tilde{p}[j] \right|
            \leq \sqrt{\tfrac{4p[j] \log\left( \frac{d}{\beta} \right)}{m_1}}
        $.
    \end{clm}
    
    \begin{clm}[Sampling Error for Small Coordinates in Final Round]\label{clm:final-samp-err-sml}
        For each $j \in S_F$, such that $p_j \leq \frac{1}{d}$,
        with probability at least $1-2\beta/d$,
        we have,
        $
        \left| p[j] - \tilde{p}[j] \right|
        	\leq \frac{\alpha}{8d}
        $.
    \end{clm}
    
    \begin{clm}[No Truncation in Final Round]\label{clm:final-no-trunc}
        With probability at least $1-\beta$,
        for every $Y^{F}_{i}
        \in Y^{F}$, $\abs{Y^{F}_{i}} \leq B_{F}$,
        so no rows of $Y^{F}$ are truncated in the
        computation of $\tmean_{B_{F}}(Y^{F})$.
    \end{clm}
    
    \begin{clm}[Error due to Privacy in Final Round]\label{clm:final-priv-err}
    With probability at least $1-2\beta$,
    $
    \forall j \in S_{r}~~\left| \tilde{p}[j] - q_{r}[j] \right| \leq
    \tfrac{4\log\left(\frac{m_1}{\beta}\right)\log\left(\frac{d}{\beta}\right)}{\eps m_1}
    $.
    \end{clm}

    Note that because no truncation happens in this round,
    the sampling error without the Laplace noise is
    bounded by the quantity as specified in
    Claims~\ref{clm:final-samp-err-lrg}
    and~\ref{clm:final-samp-err-sml}. Because of the
    possible difference in magnitudes of the means
    of the marginals in $S_F$, we establish their error
    guarantees separately. Let $H \subset S_F$ be the
    set of all coordinates, whose means are greater
    than $\tfrac{1}{d}$, i.e.,
    $H \coloneqq \{j \in S_F: p[j] > 1/d\}$.
    Likewise, let $L \subseteq S_F$ be the set of lighter
    coordinates, i.e., $L \coloneqq S_F \setminus H$.

    We analyse the heavier coordinates in $H$ first. Let
    $\wt{P}[H]$ be the product distribution over the
    coordinates in $H$ with mean $\tilde{p}[H]$.
    For all $j \in H$, using Claim~\ref{clm:final-samp-err-lrg}
    and our choice of $m_1$, we know that
    $$\abs{\tilde{p}[j]-p[j]} \leq \sqrt{\frac{4p[j] \log\left( \frac{d}{\beta} \right)}{m_1}} \implies \frac{4(p[j]-\tilde{p}[j])^2}{p[j]} \leq \frac{16\log\left(\frac{d}{\beta}\right)}{m_1} \leq \frac{\alpha^2}{32d},$$
    which (by Lemma~\ref{lem:chi-ub}) means that
    $\dcs(\wt{P}[j],P[j]) \leq \tfrac{\alpha^2}{32}$.
    Combined with Lemma~\ref{lem:pinsker}, this implies
    that $\dtv(P[j],\wt{P}[j]) \leq \tfrac{\alpha}{8d}$.
    Now, from Claim~\ref{clm:final-priv-err} and our choice
    of $m_1$, we know that for all $j \in H$,
    $$\abs{\tilde{p}[j]-q[j]} \leq \frac{4\log\left(\frac{m_1}{\beta}\right)\log\left(\frac{d}{\beta}\right)}{\eps m_1} \leq \frac{\alpha}{8d},$$
    which implies that
    $\dtv(\wt{P}[j],Q[j]) \leq \tfrac{\alpha}{8d}$.
    Therefore, by triangle inequality,
    $\dtv(P[j],Q[j]) \leq \tfrac{\alpha}{4d}$. Finally,
    from Lemma~\ref{lem:sd-ub}, we have that
    $\dtv(P[H],Q[H]) \leq \tfrac{\alpha}{4}$.

    Next, we bound the error on the lighter coordinates
    in $L$. Claims~\ref{clm:final-samp-err-sml}
    and~\ref{clm:final-priv-err}, the triangle inequality,
    and our choice of $m_1$ show that for all $j \in L$,
    \begin{align*}
        \abs{p[j]-q[j]} \leq \frac{\alpha}{8d} + \frac{4\log\left(\frac{m_1}{\beta}\right)\log\left(\frac{d}{\beta}\right)}{\eps m_1}
            \leq \frac{\alpha}{8d} + \frac{\alpha}{8d}
            = \frac{\alpha}{4d}.
    \end{align*}
    This implies that for all $j \in L$,
    $\dtv(P[j],Q[j]) \leq \tfrac{\alpha}{4d}$.
    Therefore, from Lemma~\ref{lem:sd-ub},
    $\dtv(P[L],Q[L]) \leq \tfrac{\alpha}{4}$.

    Finally, through an application of Lemma~\ref{lem:sd-ub}
    again, we obtain that
    $\dtv(P[S_F],Q[S_F]) \leq \dtv(P[H],Q[H]) + \dtv(P[L],Q[L]) \leq \tfrac{\alpha}{2}$.
    This completes our proof.
\end{proof}

\subsubsection{Putting It All Together}

In this section, we combine Lemmata~\ref{lem:ppde_partitioning} and~\ref{lem:ppde_final} to prove Proposition~\ref{thm:ppde_acc}. First, by Lemma~\ref{lem:ppde_partitioning}, with probability at least $1-O(\beta)$, if $S_{P}$ is the set of coordinates $j$, such that $q[j]$ was set in any of the partitioning rounds, then, 
\begin{enumerate}
\item $\SD(P[S_{P}], Q[S_{P}]) \leq \tfrac{\alpha}{2}$ and
\item if $j \not\in S_{F}$ and $k$ is the index of the final round, then $p[j] \leq u_{k}$ and $u_{k}\abs{S_F} < 1$.
\end{enumerate}
Next, due to the second consequence listed above, we can apply Lemma~\ref{lem:ppde_final} to obtain that if $S_{F}$ consists of all coordinates set in the final round, then with probability at least $1-O(\beta)$, $\SD(P[S_{F}], Q[S_{F}]) \leq \tfrac{\alpha}{2}$. Finally, we use the union bound and Lemma~\ref{lem:sd-ub} to conclude that, with probability at least $1-O(\beta)$,
$$
    \SD(P,Q) \leq \SD(P[S_{P}], Q[S_{P}]) + \SD(P[S_{F}], Q[S_{F}]) \leq \alpha.
$$
This completes the proof of Proposition~\ref{thm:ppde_acc}.
